Churn Reduction via Distillation

In real-world systems, models are frequently updated as more data becomes available, and in addition to achieving high accuracy, the goal is to also maintain a low difference in predictions compared to the base model (i.e. predictive "churn"). If model retraining results in vastly different behavior, then it could cause negative effects in downstream systems, especially if this churn can be avoided with limited impact on model accuracy. In this paper, we show an equivalence between training with distillation using the base model as the teacher and training with an explicit constraint on the predictive churn. We then show that distillation performs strongly for low churn training against a number of recent baselines on a wide range of datasets and model architectures, including fully-connected networks, convolutional networks, and transformers.

==> backup-notes.tex <==
\subsection{Proof of Theorem \ref{thm:opt-feasibility}}
\label{app:proof-opt-feasibility}
We first note that because $\|\phi(\z)\|_\infty < B, \forall \z \in \Delta_m$, both $\hat{R}(h) < B$ and $\hat{C}(h) < B$. Also, because $\phi$ is convex, both $\hat{R}(h)$ and $\hat{C}(h)$ are convex in $h$.
Furthermore, the objective in \eqref{eq:h-lambda} can be decomposed into a convex combination of the empirical risk and churn:
\begin{eqnarray*}
    \hat{\cL}_\lambda(\h) &=&
    \frac{1}{n}\sum_{i=1}^n (\lambda\e_{y_i} + (1-\lambda)\g(x_i))\cdot \phi(\h(x_i))\nonumber\\
    &=& \lambda\hat{R}(\h) \,+\, (1-\lambda)\hat{C}(\h) +  \frac{1}{n}\sum_{i=1}^n\g(x_i)\cdot \phi(\g(x_i)).
\end{eqnarray*}
Therefore minimizing $\hat{\cL}_\lambda(\h)$ is equivalent to minimizing the Lagrangian function 
$$\hat{R}(\h) \,+\, \mu(\hat{C}(\h) - \epsilon)$$ over $\h$
for $\mu = \frac{1-\lambda}{\lambda}$. Moreover, because each $\h_k$ minimizes $\hat{\cL}_{\lambda_k}(\h)$ for a $\lambda_k \in \Lambda$, we have that equivalently, each $\h_k$ minimizes $\hat{R}(\h) \,+\, \mu_k(\hat{C}(\h) - \epsilon),$ where $\mu_k = \frac{1-\lambda_k}{\lambda_k}$.

Before proceeding to prove Theorem \ref{thm:opt-feasibility}, we state and prove a couple of useful lemmas.
%Recall $\hat{\h}$ is the classifier returned by Algorithm \ref{alg:churn-distil} for the specified choice of $\Lambda$.
\begin{lem}
Let the scoring function $\phi: \Delta_m \> \R_+^m$ be convex, and let $\|\phi(\z)\|_\infty < B, \forall \z \in \Delta_m$. Let $\cF$ be a convex set of classifiers which includes a classifier $\g$. 
Let $\tilde{\f}$ be an optimal feasible classifier in $\cF$, i.e. $C(\tilde{\f}) \leq \epsilon$ and $R(\tilde{\f}) \leq R(\f)$ for all classifiers $\f \in \cF$ for which $C(\f) \leq \epsilon$. Then there exists a \emph{bounded} Lagrange multiplier $\tilde{\mu} \in [0, B/\epsilon]$ such that $(\tilde{\f}, \tilde{\mu})$ is a saddle point for the Lagrangian ${R}(\f) \,+\, \mu({C}(\f) - \epsilon)$:
\begin{equation*}
    \max_{\mu \in [0, 2B/\epsilon]}{R}(\tilde{\f}) \,+\, \mu({C}(\tilde{\f}) - \epsilon) \,\leq \min_{\f \in \cF}{R}(\f) \,+\, \tilde{\mu}({C}(\f) - \epsilon).
    \label{eq:minmax}
\end{equation*}
\end{lem}
\begin{lem}
Let $\hat{\h}$ be the classifier returned by Algorithm \ref{alg:churn-distil} when  $\Lambda$ is set to $\big\{\frac{1}{1 + \mu} \,\big|\, \mu \in M\big\}$ where $M=\big\{0, \frac{2B}{\epsilon(L-1)}, \frac{4B}{\epsilon(L-1)}, \ldots, \frac{2B}{\epsilon}\big\}$ for some $L \in \N_+$. Fix $\delta \in (0,1)$. 
Suppose $R$ and $C$ satisfy the generalization bounds in Theorem \ref{thm:opt-feasibility} with error bounds $\Delta_R(n,\delta)$ and $\Delta_C(n,\delta)$ respectively. Then there exists a \emph{bounded} Lagrange multiplier $\hat{\mu} \in [0, 2B/\epsilon]$ such that $(\hat{\h}, \hat{\mu})$ is an approximate saddle point for the Lagrangian ${R}({\h}) \,+\, \mu({C}({\h}) - \epsilon)$, i.e.\ w.p. $\geq 1-\delta$ over draw of sample $S \sim D^n$,
\begin{eqnarray*}
    \lefteqn{\max_{\mu \in M} {R}(\hat{\h}) \,+\, \mu({C}(\hat{\h}) - \epsilon) \,\leq\, \min_{\h\in \cH} {R}(\h) \,+\, \hat{\mu}({C}(\h) -\epsilon)}\\
    &&\hspace{4cm}\,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big).
\end{eqnarray*}
\label{lem:min-max-equivalence}
\end{lem}
\begin{proof}
Note that the classifier $\hat{\h}$ returned by Algorithm \ref{alg:churn-distil} is a solution to:
\[
\min_{\h \in \co(\h_1, \ldots, \h_L,\g)}\hat{R}(\h)~~\text{s.t.}~~\hat{C}(\h) \leq \epsilon
\]
Applying Lemma \ref{lem:min-max-equivalence} to the hypothesis class $\co(\h_1, \ldots, \h_L,\g)$, we have that there exists $\tilde{\mu} \in [0, B/\epsilon]$ such that such that $(\hat{\h}, \tilde{\mu})$ is a saddle point for the Lagrangian ${R}(\h) \,+\, \mu({C}(\h) - \epsilon)$:
\[
\max_{\mu\in [0, 2B/\epsilon]} \hat{R}(\hat{\h}) \,+\, \mu (\hat{C}(\h) - \epsilon) \,\leq\, \min_{\h \in \co(\h_1,\ldots, \h_{L}, \g)} \hat{R}(\h) \,+\, \tilde{\mu} (\hat{C}(\h) - \epsilon).
\]
We denote by $M = \{0, \frac{2B}{\epsilon(L-1)}, \ldots, \frac{2B}{\epsilon}\}$ a discretization of the space of multipliers. Allowing  
$\hat{\mu}$ to denote closest value to $\tilde{\mu}$ in this set, we have that:
\begin{eqnarray}
\max_{\mu \in M} \hat{R}(\hat{\h}) \,+\, \mu (\hat{C}(\h) - \epsilon) 
&\leq& \min_{\h \in \co(\h_1,\ldots, \h_{L}, \g)} \hat{R}(\h) \,+\, \hat{\mu} (\hat{C}(\h) - \epsilon) \,+\, \frac{2B^2}{\epsilon(L-1)}
\nonumber
\\
&=& \min_{\h \in \cH} \hat{R}(\h) \,+\, \hat{\mu} (\hat{C}(\h) - \epsilon) \,+\, \frac{2B^2}{\epsilon(L-1)},
\label{eq:min-max-empirical}
\end{eqnarray}
where the last step follows from the fact that $\co(\h_1,\ldots, \h_{L}, \g) \subseteq \cH$ and each $\h_k$ was chosen to minimize $\hat{R}(\h) \,+\, \mu_k (\hat{C}(\h) - \epsilon)$  for a $\mu_k \in M$. 

For a fixed $\mu \in M$, we can apply the generalization bounds for $R$ and $C$ and have w.p. $\geq 1-\delta$ over draw of sample $S \sim D^n$:
\[
\big|\big(\hat{R}(\h) + \mu(\hat{C}(\h) - \epsilon)\big) \,-\, \big({R}(\h) \,+\, {\mu} ({C}(\h) - \epsilon)\big)\big| \,\leq\,
\Delta_R\left(n,\delta\right) \,+\, \frac{2B}{\epsilon}\Delta_C\left(n,\delta\right).
\]
Taking a union bound over over all $L$ multiplier values in $M$, and plugging the bound  back into \eqref{eq:min-max-empirical} completes the proof.
%
% Let $\hat{\mu} = \frac{1 - \hat{\lambda}}{\hat{\lambda}}$, where $\hat{\lambda}$ the mixing parameter chosen by Algorithm \ref{alg:churn-distil}. Then
% its easy to see that $\hat{\mu}$ solution to
% % \[
% % \min_{\h \in \{\h_1,\ldots, \h_{L+1}\}}\, \hat{R}(\h) ~~~\text{s.t.}~~~ \hat{C}(\h) \leq \epsilon.
% % \]
% % Equivalently, this can be written as:
% \[
% \hat{\mu} \in \underset{\mu \in \{0, B/L\epsilon, \ldots, B/\epsilon\}}{\argmax}\min_{\h \in \cH} \hat{R}(\h) \,+\, \mu(\hat{C}(\h) - \epsilon).
% \]
% Furthermore,
% $\hat{\h} \in \argmin_{\h \in \cH} \hat{R}(\h) \,+\, \hat{\mu}(\hat{C}(\h) - \epsilon)$.
% Because 
% $\phi$ is convex, $\hat{R}(\h)$ and $\hat{C}(\h)$ are convex in $\h$. Therefore there exists a $\hat{\mu} \in \R_+$ such that $(\hat{\mu}, \hat{\h})$ forms a pure Nash equilibrium:
% \[
% \max_{\mu\geq 0} \hat{R}(\hat{\h}) \,+\, \mu (\hat{C}(\h) - \epsilon) \,\leq\, \min_{\h \in \co(\h_1,\ldots, \h_{L+1})} \hat{R}(\h) \,+\, \hat{\mu} (\hat{C}(\h) - \epsilon).
% \]
\end{proof}

We are now ready to prove Theorem \ref{thm:opt-feasibility}.
\begin{proof}[Proof of Theorem \ref{thm:opt-feasibility}]
Combining Lemma \ref{lem:min-max-equivalence} that
\begin{equation}
    \max_{\mu \in M} {R}(\hat{\h}) \,+\, \mu({C}(\hat{\h}) - \epsilon) \,\leq\, \min_{\h\in \cH} {R}(\h) \,+\, \hat{\mu}({C}(\h) -\epsilon) \,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big).
    \label{eq:approx-saddle-point}
\end{equation}
To show optimality, lower bound the LHS in \eqref{eq:approx-saddle-point} by setting $\mu = 0$ and upper bound the RHS by setting $\h$ to the optimal feasible solution $\tilde{\h}$, giving us:
\[
{R}(\hat{\h}) \,\leq\,{R}(\tilde{\h}) + \hat{\mu}(0) \,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big),
\]
as desired. 

To show feasibility, we first apply Lemma \ref{lem:min-max-equivalence} to the hypothesis class $\cH$, and have that there exists a $\tilde{\mu} \in [0, \frac{B}{\epsilon}]$ such that 
\begin{equation*}
\min_{\h \in \cH}{R}(\h) \,+\, \tilde{\mu}({C}(\h) - \epsilon) \geq
    \max_{\mu \in [0, 2B/\epsilon]}{R}(\tilde{\h}) \,+\, \mu({C}(\tilde{\h}) - \epsilon),
\end{equation*}
which can be lower bounded by setting $\mu = 0$, giving us:
\begin{equation}
\min_{\h \in \cH}{R}(\h) \,+\, \tilde{\mu}({C}(\h) - \epsilon) \geq {R}(\tilde{\h}).
\label{eq:min-max-lower-bound}
\end{equation}
We next  lower bound the LHS of \eqref{eq:approx-saddle-point} by setting $\mu = \tilde{\mu} \,+\, \frac{B}{\epsilon}$ and upper bound the RHS of \eqref{eq:approx-saddle-point} by setting $\h$ to the optimal feasible solution $\bar{\h}$:
\begin{eqnarray*}
 {R}(\hat{\h}) \,+\, \tilde{\mu}({C}(\hat{\h}) - \epsilon) \,+\, \frac{B}{\epsilon}({C}(\hat{\h}) - \epsilon) &\leq& 
R(\tilde{\h}) \,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big).
\end{eqnarray*}
We next lower bound the first two terms in the LHS by taking a min over $\h \in \cH$:
\begin{eqnarray*}
\min_{\h \in \cH} \left\{{R}({\h}) \,+\, \tilde{\mu}({C}({\h}) - \epsilon)\right\} \,+\, \frac{B}{\epsilon}({C}(\hat{\h}) - \epsilon) &\leq& 
R(\tilde{\h}) \,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big),
\end{eqnarray*}
and use \eqref{eq:min-max-lower-bound} to further lower bound the min over $\h \in \cH$ with $R(\tilde{\h})$:
\[
R(\tilde{\h}) \,+\, 
\frac{B}{\epsilon}({C}(\hat{\h}) - \epsilon) \,\leq\,
R(\tilde{\h}) \,+\, \textstyle\cO\Big(\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{\epsilon}\Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B^2}{L\epsilon}\Big).
\]
% and we further have:
% \[
% {C}(\hat{\h}) \leq \epsilon \,+\, \textstyle\cO\Big(\frac{\epsilon}{B}\Delta_R\left(n,\frac{\delta}{L}\right) \,+\, \Delta_C\left(n,\frac{\delta}{L}\right) \,+\, \frac{B}{L}\Big)
% \]
Rearranging the terms gives us the desired feasibility result.
\end{proof}

\subsection{Proof of Proposition \ref{prop:risk-churn-bound}}
\label{app:proof-risk-churn-bound}
\begin{proof} 
Expanding the classification risk in terms of the class probability function $\p$, we have:
\begin{eqnarray*}
\lefteqn{{R}(\hat{\h}) \,-\, {R}(\tilde{\h})}\\
&=& \E_{x\sim D_\X}\left[\E_{y|x}\left[\e_y\cdot\phi(\hat{\h}(x))\right]\right] \,-\, \E_{x\sim D_\X}\left[\E_{y|x}\left[\e_y\cdot\phi(\tilde{\h}(x))\right]\right]\\
&=& \E_{x\sim D_\X}\left[\p(x)\cdot\phi(\hat{\h}(x))\right] \,-\, \E_{x\sim D_\X}\left[\p(x)\cdot\phi(\tilde{\h}(x))\right]\\
&\leq& \E_{x\sim D_\X}\left[\p(x)\cdot\left(\phi(\hat{\h}(x)) -   \phi(\g(x))\right)\right] \,+\, \Phi\E_{x\sim D_\X}\left[\|\tilde{\h}(x) - \g(x)\|_1\right]\\
&\leq& \E_{x\sim D_\X}\left[\g(x)\cdot\left(\phi(\hat{\h}(x))-   \phi(\g(x))\right)\right]
 \,+\, B\E_{x\sim D_\X}\left[\|\p(x) - \g(x)\|_1\right] \,+\, \Phi\E_{x\sim D_\X}\left[\|\tilde{\h}(x) - \g(x)\|_1\right],
\end{eqnarray*}
where the second step follows from the Lipschitz property and the last step follows from the boundedness assumption on $\phi$.
\end{proof}


\begin{lem}
Let the scoring function $\phi: \Delta_m \> \R_+^m$ be convex, and let $\|\phi(\z)\|_\infty < B, \forall \z \in \Delta_m$. Let $\cF$ be a convex set of classifiers which includes a classifier $\f$ for which $\hat{C}(\f) = 0$.
Let $\tilde{\f}$ be an optimal feasible classifier in $\cF$, i.e. $\hat{C}(\tilde{\f}) \leq \epsilon$ and $\hat{R}(\tilde{\f}) \leq \hat{R}(\f)$ for all classifiers $\f \in \cF$ for which $\hat{C}(\f) \leq \epsilon$. Then there exists a \emph{bounded} Lagrange multiplier $\tilde{\lambda} \in [\frac{\epsilon}{\epsilon+B}, 1]$ such that $(\tilde{\f}, \tilde{\mu})$ forms an equilibrium of the Lagrangian min-max game: %is a saddle point for the Lagrangian ${R}(\f) \,+\, \mu({C}(\f) - \epsilon)$:
\begin{equation*}
    %\max_{\mu \in [0, 2B/\epsilon]}{R}(\tilde{\f}) \,+\, \mu({C}(\tilde{\f}) - \epsilon) \,\leq \min_{\f \in \cF}{R}(\f) \,+\, \tilde{\mu}({C}(\f) - \epsilon).
    \tilde{\lambda}\hat{R}(\tilde{\f}) \,+\, (1-\tilde{\lambda})(\hat{C}(\tilde{\f}) - \epsilon) \,=\,
    \min_{\f \in \cF}\tilde{\lambda}\hat{R}(\f) \,+\, (1-\tilde{\lambda})(\hat{C}(\f) - \epsilon)
\end{equation*}
\begin{equation*}
    %\max_{\mu \in [0, 2B/\epsilon]}{R}(\tilde{\f}) \,+\, \mu({C}(\tilde{\f}) - \epsilon) \,\leq \min_{\f \in \cF}{R}(\f) \,+\, \tilde{\mu}({C}(\f) - \epsilon).
    \max_{\lambda \in [\frac{\epsilon}{\epsilon+B}, 1]} (1-{\lambda})(\hat{C}(\tilde{\f}) - \epsilon) \,=\,
    (1-\tilde{\lambda})(\hat{C}(\tilde{\f}) - \epsilon).
\end{equation*}
\end{lem}
\begin{lem}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

